Disturbance Decoupling for Gradient-based Multi-Agent Learning with Quadratic Costs

Motivated by applications of multi-agent learning in noisy environments, this paper studies the robustness of gradient-based learning dynamics with respect to disturbances. While disturbances injected along a coordinate corresponding to any individual player's actions can always affect the overall learning dynamics, a subset of players can be disturbance decoupled---i.e., such players' actions are completely unaffected by the injected disturbance. We provide necessary and sufficient conditions to guarantee this property for games with quadratic cost functions, which encompass quadratic one-shot continuous games, finite-horizon linear quadratic (LQ) dynamic games, and bilinear games. Specifically, disturbance decoupling is characterized by both algebraic and graph-theoretic conditions on the learning dynamics, the latter is obtained by constructing a game graph based on gradients of players' costs. For LQ games, we show that disturbance decoupling imposes constraints on the controllable and unobservable subspaces of players. For two player bilinear games, we show that disturbance decoupling within a player's action coordinates imposes constraints on the payoff matrices. Illustrative numerical examples are provided.

==> TD_stuff.tex <==
% Quadratic games can also be used to model algorithms in MARL, where often a network structure is imposed on the gradient updates of individual agents. Here we show that the distributed policy evaluation problem in decentralized MARL, in which agents cooperatively agree on the value function over a communication network is a quadratic continuous game. 
% Additionally, quadratic games captures policy evaluation in MARL. 
\subsection{Gradient-based TD in distributed policy evaluation}
\label{ex:MARL}
In reinforcement learning, it is assumed that the player faces unknown stochastic (typically Markovian) dynamics and reward. Two important aspects of the reinforcement learning process are policy improvement and policy evaluation. The latter is such that the learner must evaluate the performance of a policy on an unknown environment (i.e., unknown dynamics and unknown rewards). TD is a commonly used process for policy evaluation~\cite{dann2014policy}. It has been shown that TD can be formulated as a gradient based update~\cite{sutton2018reinforcement}, and furthermore, distributed versions of TD are becoming common~\cite{zhang2018fully,doan2019finite}. We demonstrate that distributed TD corresponds to gradient-based learning in a quadratic continuous game and characterize its disturbance decoupling properties.

Facing a Markov decision process (MDP), the goal of the agents is to cooperatively find the average of the total discounted accumulative reward $J$ over the network, which is given by $J(z)=\mb{E}[\sum_{k=0}^\infty \frac{\beta^k}{N}\sum_{i\in [N]} R_i(z_k,u_k,z_{k+1})|z_0=z]$ where $R_i$ is the reward function, $u_k\in \mb{R}^m$ is such that $u_k\sim \pi(\cdot|z_k)$ and $z_k$ denotes the MDP state. State transitions are determined by the transition kernel $P:Z\times Z\rightarrow [0,1]$, whose entries we denote by $p_{ij}$ and where $Z$ is the finite state space. When the state space is large, it is common to approximate $J$ with a set of basis function: $\tilde{J}(j,\theta)=\sum_{\ell=1}^q\theta_\ell \phi_\ell(j)$ where $j\in [|Z|]$, i.e. index of the state. Let $\phi(j)=(\phi_1(j), \ldots, \phi_q(j))^\top$ and $\Phi=\begin{bmatrix}\phi(1) & \cdots & \phi(|Z|)\end{bmatrix}^\top$.
%\[\Phi=\begin{bmatrix}\text{---} & \phi(1)^\top &\text{---}\\
%\vdots & \vdots & \vdots \\
%\text{---} & \phi(|Z|)^\top %&\text{---}\end{bmatrix}.\]
Each agent $i$ maintains its own estimate $\theta_i=(\theta_{1}^i,\ldots, \theta_{q}^i) \in \mb{R}^{q}$
of the weight $\theta^\ast$, and the goal is to update their estimates of $\theta$ until the reach consensus. The  $\theta^\ast$ that best approximates $J$ is defined by $\Pi J=\Phi\theta^\ast$ where $\Pi J=\arg\min_{y\in \mathrm{span}(\phi_\ell)}\|y-J\|_{\mathrm{diag}(\pi(1), \ldots, \pi(|Z|))}$ (cf.~\cite[Sec.~2.2]{doan2019finite} for further characterization).  Player $i$ has estimate $\tilde{J}_i(\theta)=\Phi^\top \theta^i$. 

At every iteration $k \geq 0$, each
agent $i$ first performs a weighted average to combine its own estimate and the ones received from its
neighbors $j \in N_i$,
$y_{k}^i=\sum_{j\in N_i} W_{ij}\theta_{k}^j$ where $W$ is a doubly stochastic matrix and $\theta_{k}^j$ is the $j$-th players estimate at time $k$.
Each agent receives the  temporal difference $\delta_{k}^i$ based on observed data $(z_k,z_{k+1},r_{k}^i)$ returned by the environment using
\[\delta_{k}^i=r_{k}^i+(\beta \phi(z_{k+1})-\phi(z_k))^\top \theta_{k}^i.\]
Here $\delta_{k}^i$ 
represents the difference between the local outcome at agent $i$, namely $r_{k}^i+\beta \tilde{J}(z_{k+1},\theta_{k}^i)$, and the current estimate $\tilde{J}(z_k,\theta_{k}^i)$. Using $y_{k}^i$ and $\delta_{k}^i$ agent $i$ then performs a gradient update to updates its estimate $\theta^{i}$ as 
\begin{equation}\label{eqn:TD_distributedUpdate}
   \textstyle \theta_{k+1}^i=y_{k}^i+\gamma G_k \delta_{k}^i
\end{equation}
with $G_k=\sum_{\ell=0}^k(\beta \lambda)^{k-\ell}\phi(z_{\ell})$. Treating $\theta^i$, i.e. player $i$'s estimate of $\theta^\ast$, as the action $x_i$ in a game $(f_1,\ldots, f_N)$ we show that distributed TD as described above corresponds to gradient-based learning in a continuous game. 

\textcolor{red}{This is time dependent update. Suppose that
\begin{align}\label{eqn:marl_cost}
  f_i(\theta) =&   \textstyle  \half\sum_{j \in N_i} (\theta_i - \theta_j)^\top W_{ij} (\theta_i - \theta_j)\notag\\
    &   \textstyle\quad+\half\norm{\Phi \theta_i - \Phi \theta^\ast}^2_{\mc{D}}
    %- J_e(\theta_i),
\end{align}
Then,
\[D_{\theta_i}f_i(\theta_k)=\textstyle \sum_{j\in N_i} W_{ij}(\theta_{i,k}-\theta_{j,k})+\Phi^\top \Phi(\theta_{i,k}-\theta^\ast)\]
So then a gradient based update is
\begin{equation*}
 \theta_{i,k+1}=\textstyle\theta_{i,k}-\gamma (\sum_{j\in N_i} W_{ij}(\theta_{i,k}-\theta_{j,k})+\Phi^\top \Phi(\theta_{i,k}-\theta^\ast))
\end{equation*}
Now, in TD what is happening is that there is an asynchronous update going on in the sense of which rows of $\Phi$ are being selected. The matrix $\Phi\in \mb{R}^{|Z|\times q}$ is all the possible feature vectors evaluated at all the possible states. So basically in round $k$, the policy is sampled to get state $z_{k+1}, (r_k^i)_{i\in [N]}$ and we have $z_k$ our current state. Then each player computes 
\[\delta_k^i=r_k^i+(\beta \phi_{k+1}-\phi_k)^\top \theta^i\]
where $\phi_k=\phi(z_k)$. Then according to the consensus paper they update
\[\theta_{k+1}^i=y^i_k+\gamma \phi_k\delta_k^i\]
(note we could replace $\phi_k$ with $G_k$ but that additionally complicates things), but we are claiming (and you should check this numerically) that 
\begin{align}
    \theta_{k+1}^i&=\textstyle\theta_k^i-\gamma\big( \sum_{j\in N_i} W_{ij}(\theta_{k}^i-\theta_{k}^j)+\ \phi_k\delta_k^i\big)\\
    &=\textstyle\theta_k^i-\gamma\big( \sum_{j\in N_i} W_{ij}(\theta_{k}^j-\theta_{k}^j)\notag\\
    &\quad\textstyle+\ \phi_k(r_k^i+(\beta \phi_{k+1}-\phi_k)^\top \theta^i_k)\big)
\end{align}
will also converge. I think it will. This in and of it self would be an extension to the paper \cite{doan2019finite}. Now this is a gradient update in the form of this paper except its linear time varying because the input term $\phi_kr_k^i$ and and term $\beta\phi_{k+1}-\phi_k$.
}
% \textcolor{red}{@sarah: now formulate the game with this description of TD... We can choose how to shorten after getting things in...}

% In distributed policy evaluation via TD~\cite[Chp.9]{sutton2018reinforcement}, players collectively estimate the stationary value function $J^\star \in \reals^Z$ corresponding to a given policy $\pi$. Given a set of feature vectors $\Phi = [\phi_1, \ldots \phi_q]$, each player solves $\min_{\theta_i \in \reals^{q}} e_i(\theta_i)$ where $e_i$ is given by

% by performing a TD update with respect to~\eqref{eqn:MARL_objective} on the \emph{weighted average} $y_{i,k} = \sum_{j \neq i} W_{ij}{\theta}_{j,k}$. The objective~\eqref{eqn:MARL_objective} is weighted by $\mc{D}$, the stationary distribution associated with $\pi$~\cite{doan2019finite}. 
% We model distributed policy evaluation via TD as a cooperative continuous game with quadratic costs. 
\begin{proposition}
Gradient-based TD for distributed policy evaluation corresponds to gradient-based learning in a quadratic continuous game in which each player $i$ has cost 
\begin{align}\label{eqn:marl_cost}
  f_i(\theta_1, \ldots, \theta_N,k) =&   \textstyle - \half\sum_{j \neq i} (\theta_i - \theta_j)^\top W_{ij} (\theta_i - \theta_j)\notag\\
    &   \textstyle\quad-\half\norm{\Phi \theta_i - \Phi \theta^\ast}^2_{\mc{D}}
    %- J_e(\theta_i),
\end{align}
where $W_{ij} \geq 0$ denote the weight of the communication link between players $i$ and $j$, and $\mc{D}$ is the stationary distribution associated with $\pi$.
%$J_e$ is the accumulative reward approximation error weighted by , as given by
%\begin{equation}\label{eqn:MARL_objective}
%    J_e(\theta,k)= \half\norm{\sum_{\ell = 1}^{q} \theta(\ell)\phi_\ell(z_k) - J^\ast}^2_{\mc{D}}. 
%\end{equation}
\end{proposition}
\begin{proof}
Since $f_i$ is a quadratic function in $(\theta_{1,k}, \ldots, \theta_{N,k})$, it suffices to show that~\eqref{eqn:gradientUpdate} evaluates to the dynamics given by~\eqref{eqn:TD_distributedUpdate}. Let $\textstyle h_i(\theta_{1,k}, \ldots, \theta_{N,k}) = - \frac{1}{\gamma}(\sum_{j \neq i}W_{ij}(\theta_{i,k} - \theta_{j,k})) - G_{i,k} d_{i,k}$, where $-\frac{1}{\gamma}(\sum_{j \neq i} W_{ij}(\theta_{i,k} - \theta_{j,k}))$ is derived from the \textcolor{red}{partial derivative} of the first term in $f_i(\theta)$. The second term $G_{i,k} d_{i,k}$ is the TD~\cite{sutton2018reinforcement}.
The gradient-based learning dynamics~\eqref{eqn:gradientUpdate} with $h_i(\theta_{1,k}, \ldots, \theta_{N,k})$ evaluates to
\begin{equation}\label{eqn:marl_gradientUpdate}
    \theta_{i,k+1} = \textstyle (1 - \sum_{j\neq i} W_{ij})\theta_{i,k}  + \sum_{j \neq i} W_{ij}\theta_{j,k}+ \gamma G^\top_{i,k} d_{i,k}.
\end{equation} 
Since $W$ is a stochastic matrix, $1 - \sum_{j\neq i}W_{ij} = W_{ii}$, therefore $(1 - \sum_{j\neq i} W_{ij})\theta_{i,k}  + \sum_{j \neq i} W_{ij}\theta_{j,k} = y_k^i$, and we recover the distributed policy evaluation update given in~\eqref{eqn:TD_distributedUpdate}. 
% Since $G_{i,k}^\top d_{i,k}$ is a stochastic approximation, it varies at each learning iteration $k$. 
More generally, \eqref{eqn:marl_gradientUpdate} is a decentralized gradient method where players converge to a consensus protocol $\theta^\star= \theta_i = \theta_j$ which minimizes $\frac{1}{N}\sum_{i \in [N]} f_i(\theta)$~\cite{nedic2018network}.
\end{proof}
\textcolor{Blue}{A couple things. Does this update even converge to the correct $\theta^\ast$? You have added an additional term $\theta_{i,k}$ and I am not sure if that will converge. Looking back at the red above in particular the equation
\[\theta_{k+1}^i=y_{k}^i+\gamma\phi_k\delta_k^i\]
My suggestion is to write a positive results. (so first note that this is different than (15) and we replaced $G_k$ which is discounted to just $\phi_k$ to make it simple). The result will have the following claims:}
\begin{itemize}
    \item \textcolor{Blue}{TD for policy evaluation given linear function approximation representation of the value function $J$ is a linear system with an "affine disturbance term"
    \item Treating this affine disturbance term $\gamma \phi_k\delta_k^i$ as the disturbance, we can prove that this system is never disturbance decoupled}
    \item \textcolor{Blue}{This is a positive result because you want the individually observed rewards $r_k^i$ and the other agents estimates of the value $J$ (which is what $\delta_k^i$ approximates, i.e. the TD of the reward) to propagate through this system in order to ensure we get consensus.}
    \item \textcolor{Blue}{Then propose that designing the the $W_{ij}$ matrix (which is like the cost agent $i$ places on the difference between player $i$'s estimate and player $j$'s can aid in improving convergence. Q: is there a way to characterize the effect of for example a large reward at player $i$ or a large estimation error $\theta_i-\theta^\ast$ (which comes in as the input) and the effects it has (through this path/graph kind of analysis) on the other states? Maybe you can explore this in your simple little example 2 below. And just show that }
\end{itemize}
\textcolor{Blue}{If we cant make this sound reasonable, we should drop this TD stuff until we can handle TV things, and just add in a different class of games, in particular you can use simgrad and altgrad as examples of learning dynamics in bilinear games (see citations I provided in slack). I think that is probably going to be what we should do since your results for this game are super weak. You just have a toy example which is not informative in Example 2. I thought we had results on potential and zero sum games? where did those go? }

\textcolor{Blue}{A final note (3/14 @ 10:33. Just remove the TD stuff since there are lots of problems with it... Specially now that I see your example. You should add in simgrad and Altgrad for bilinear games. }
% When the state space is large, the set of weighted basis functions $\Phi(1), \ldots, \Phi(d)$ is used to linearly approximate $J^\star(s)$. Each individual agent uses value function approximation (VFA) to solve the minimization problem
% \begin{align}
%     \min_{\theta_i \in \reals^{d}} f_i(\Theta) = \norm{J^\star - \Phi\frac{1}{N}\sum_{i = 1}^N\theta_i}^2_D,
% \end{align}
% where $D = \diag \{y_1, \ldots, y_{|\mc{S}|}\}$ denotes the diagonal matrix weighted by the stationary distribution $y$ corresponding to $\pi$, and $\theta_i \in \reals^d$ denotes the weight parameter of agent $i$. We denote the total vector weighting vectors by $\Theta = (\theta_1, \ldots, \theta_N)$.   
% In particular, agents utilize gradient-descent dynamics over a communication network, given by
% \[\Theta^+ = W\Theta + \bar{\alpha}\diag(D_{1}f(\Theta), \ldots, D_{N}f(\Theta)),\]
% where $\bar{\alpha}$ is the step-size of the update each agent.  Here, the strategy of each agent is $\theta_i$, and the strategy space is $\mc{X}_i = \reals^d$. $W  \in \reals^{|\mc{S}|d\times|\mc{S}|d}$ denotes a communication network whose stationary distribution $\Theta^\star = (\theta_{s_1}, \ldots, \theta_{s_{|\mc{S}|}})$ is given by $\theta_s = \theta_{s'}$ forall $s \neq s'$.
 

\textbf{Distributed Policy Evaluation Game Graph}. \label{ex:MARL_gameGraph}
The game graph corresponding to~\eqref{eqn:marl_gradientUpdate} is given by $\hat{W}^k = W \otimes I_q + \gamma \diag\{G^\top_{1,k} d_{1,k}, \ldots, G^\top_{N,k} d_{N,k}\})$, where $W$ is the weighted communication adjacency matrix for distributed policy evaluation. 
Since $G^\top_{N,k} d_{N,k}$ varies at each $k$, $\hat{W}^k$ is a time varying game graph. When diminishing step sizes are used, $\lim_{k\rightarrow \infty} \hat{W}^k = W \otimes I_{q}$. Standard assumptions for convergence of gradient-based TD updates in distributed policy evaluation require \emph{doubly stochasticity} ($\lim_{k\rightarrow\infty}\hat{W}^k = \frac{\ones\ones^\top}{N}$) and element-wise non-negativity ($W_{ij} \geq 0$)~\cite{nedic2018network}.

% \subsection{Connection to consensus networks}
% The consensus protocol has many applications including distributed optimization and multi-agent reinforcement learning (MARL)~\cite{doan2019finite}. We analyze the consensus protocol as a quadratic game--- i.e. for player strategy $x_i \in \reals^n$, each player minimizes its cost function $f_i(x) = \half \sum_{j \neq i} (x_i - x_j)^TL_{ij}(x_i - x_j)$, where $L_{ij} \in \reals$ corresponds to the weights between player $i$ and player $j$ on a consensus network, and $L \in \reals^{N\times N}$ forms the \emph{weighted Laplacian} of an undirected connected graph~\cite{mesbahi2010graph}. 

% We consider the time-invariant part of MARL game graph from Example~\ref{ex:MARL_gameGraph}: $(I - L \otimes I_{n})$. 
% When the weighted graph Laplacian $L$ is positive semidefinite with exactly one zero eigenvalue,  $W$ is doubly stochastic. This results in~\eqref{eqn:marl_gradientUpdate} converging to the consensus value --- i.e. $x_i = x_j$ for all $i, j \in [N]$. 
% Although most consensus networks assume $L_{ij} \geq 0$ for all $i, j \in [N]$, this is not a necessary condition for positive semidefiniteness of $L$. In~\cite{zelazo2014definiteness}, the authors showed there exists a negative threshold $-R$, $R > 0$, such that if $L_{ij} \textgreater -R$, \eqref{eqn:consensusDym} converges to consensus. When $L_{ij} < -R$, \eqref{eqn:consensusDym} results in strategies that diverge  to infinity.

% However, we note that when $L_{ij} = -R$, \eqref{eqn:consensusDym} is still \emph{stable}, albeit $x_i \neq x_j$. We observe here that instead of consensus, $L_{ij} = -R$ turns~\eqref{eqn:consensusDym} into a disturbance decoupled network.
\begin{example}[Disturbance decoupled distributed policy evaluation]
From Section~\ref{ex:MARL_gameGraph}, the game graph in the limit of diminishing step-sizes for each player---i.e., $\lim_{k\rightarrow \infty} \gamma_i = 0, \ \forall \ i \in [N] $---is given by $W\otimes I_q$. For a four player policy evaluation game whose game graph is given by Figure~\ref{fig:DD_example}, $W\otimes I_q$ evaluates to
\[\begin{bmatrix}
1 - (\alpha + \beta) & \alpha & \beta & 0 \\ 
\alpha & 1 - (\alpha + \gamma) & 0 & \gamma \\ 
\beta & 0 & 1 - (\beta + \delta) & \delta \\
0 & \textcolor{red}{\gamma} & \delta & 1 - (\gamma + \delta)
\end{bmatrix}, \]
where given values $\alpha, \beta > 0$ such that $\alpha + \beta < 1$ is satisfied, disturbance decoupling criteria from Example~\ref{ex:DD_4Players} require $\gamma = \frac{\alpha + \beta}{2} + \half \sqrt{\alpha^2 + \beta^2 + 6\alpha\beta}$ and $\delta = -\frac{\alpha\beta}{\gamma}$. The resulting game graph given by $W$ is no longer a doubly stochastic matrix --- players will not converge to the same approximation of $J^\star$. However, we observe that for any $\delta > -\frac{\alpha\beta}{\gamma}$, $\lim_{k\rightarrow\infty} \hat{W}^k = \frac{\ones \ones^\top}{4}$, and at exactly $\delta = -\frac{\alpha\beta}{\gamma}$, the condition $\lim_{k\rightarrow\infty} \hat{W}^k = \frac{\ones \ones^\top}{4}$ fails. 

The first observation implies that requiring $W_{ij} \geq 0$ is not necessary for player consensus. This correlates well with previous observations that negative edge weights may result in the \emph{fastest} distributed averaging networks constrained to a graph structure~\cite{xiao2004fast}. The second condition implies that distributed averaging graphs and disturbance decoupled graphs are closely related yet \emph{mutually exclusive} --- i.e. a game graph cannot have both properties at the same time. 

% However, 
% In the game graph  there exists a negative threshold $-R$, $R > 0$, such that if $L_{ij} \textgreater -R$, \eqref{eqn:consensusDym} converges to consensus. When $L_{ij} < -R$, \eqref{eqn:consensusDym} results in strategies that diverge  to infinity.
% Without $\delta$, $R_{34} = \frac{-\alpha\beta\gamma}{\alpha\beta + \alpha\gamma + \beta\gamma}$ is as derived in~\cite{zelazo2014definiteness}. For any $-\delta > -R_{34}$, the dynamics given by~\eqref{eqn:consensusDym} converges to the consensus value $\frac{1}{4}\sum_{i \in [4]} x^0_i$. However when $-\delta = -R_{34}$, it can be checked numerically and analytically that $\alpha\gamma + \beta\delta$ satisfies the disturbance decoupling condition derived in Example~\ref{ex:DD_4Players}. 
\end{example}

% The connection between consensus networks and disturbance decoupling networks suggests although consensus networks converges to the consensus value of the game, it is not very robust, and that we can trade off converge to consensus value for robustness of the learning dynamics to individual gradient noise. 
% In addition to providing insights like Corollary~\ref{cor:lqGame_DD}, Theorem~\ref{thm:disturbanceDecoupling} also allows for the direct observation that the distributed MARL policy evaluation problem is always \emph{disturbance coupled} for every pair of players $(i,j)$. 
% \begin{corollary}\label{cor:marl_DD}
% In a game such as distributed MARL policy evaluation (Example~\ref{ex:MARL}), where the dynamics are given by 
% \[\Theta^+ = W\Theta + \bar{\alpha}\diag(\nabla_{\theta}f(\theta_1), \ldots, \nabla_{\theta}f(\theta_1)). \]
% Disturbance decoupling is not possible for any pair of players $(i,j)$. 
% \end{corollary}
% \begin{proof}
% Given the learning dynamics as well as the communication network, Theorem~\ref{thm:disturbanceDecoupling} states that for two players $i$ and $j$ to be disturbance decoupled, the sum of path weights of length $k$ must satisfy $\sum_{p \in \mc{P}^{ij}_k} w_{jv_1}\ldots w_{v_{k-2}i} = 0$. 

% Assuming players $(i,j)$ are connected by at least one path $p$, we note that the disturbance decoupling condition implies there must be a path $\bar{p}$ with a \emph{negative} path weight. Furthermore, this implies that there exists at least one communication link between two players $w_{ij} < 0$.
% \end{proof}
% Corollary~\ref{cor:marl_DD} suggests that to improve robustness of agents in MARL to noise in the gradient, communication networks where adversarial communication link $w_{ij} < 0$ should be allowed, such that during each consensus step, player $i$ wants to deviate from player $j$'s current strategy $\theta_j$ rather than converge to it. Such behaviour is again counter-intuitive to the goal of the consensus network, in which a team of players cooperative determine the optimal strategy of a game. In most distributed MARL policy evaluation literature, $w_{ij} \geq 0$ is always assumed. 

% However, we note that quite a substantial set of communication networks which satisfy the doubly stochastic matrix condition have adversarial links; given a network structure, the \emph{fastest} consensus rates often include negative weights~\cite{xiao2004fast}. Here we've also shown that communication networks with negative weights may also have improved robustness to gradient disturbances. Therefore it may be beneficial to consider such networks when stability of a subset of agents against input gradient noise is important. 

==> bilinearGames.tex <==
\subsection{Two player bilinear games}~\label{ex:zeroSumGame}
Bilinear games are an important class of games that have seen a resurgence in machine learning~\cite{balduzzi2018re,balduzzi2020smooth}. 
%An example application is adversarial learning, where the competition in Generative Adversarial Networks is captured by a hidden bilinear structure~\cite{vlatakis2019poincare,bailey2019finite}. 
%A two player bilinear game is defined by a pair of matrices $(A,B)$, such that player 1 seeks to minimize $x_2^\top A x_1$, and player 2 seeks to minimize $x_2^\top B x_1$. 

Hence, two player bilinear games are clearly quadratic continuous games. Gradient-based learning algorithms such as simultaneous gradient descent or alternating gradient descent are commonly studied approaches to learning in such games~\cite{vlatakis2019poincare,bailey2019finite}. We show that both simultaneous and alternating gradient play correspond to gradient-based learning dynamics given in~\eqref{eqn:gradientUpdate} and derive their game graph.

\noindent\textbf{Game graph for simultaneous gradient play.} 
Players update their actions simultaneously by following the gradient of their own cost with respect to their own action, given by
\begin{equation}\label{eqn:simGrad_update}
\begin{aligned}
\textstyle x^{k+1}_1 & = x_1^k  - \gamma_1 A^\top x^k_2 \\
x^{k+1}_2 & = x_2^k - \gamma_2 B x^k_1
\end{aligned}
\end{equation} 
The simultaneous gradient play game graph is defined by
\begin{equation}\label{eqn:simGrad_gameGraph}
    W_s = \begin{pmatrix} 
        I_{n_1} & -\gamma_1 A^\top \\
        -\gamma_2 B & I_{n_2}
    \end{pmatrix}
\end{equation}
\textbf{Game graph for alternating gradient play.} Players update their actions \emph{sequentially} by following the gradient of their cost \emph{after} the most recent action update. This is given by 
\begin{equation}\label{eqn:algGrad_update}
\begin{aligned}
      x_1^{k+1} &=\textstyle  x_1^k - \gamma_1 A^\top x^k_2\\
      x_2^{k+1} &=\textstyle x_2^k - \gamma_2 B x_1^{k+1}  
\end{aligned}
\end{equation}
The alternating gradient play game graph is defined by
\begin{equation}\label{eqn:altGrad_gameGraph}
    W_a = \begin{pmatrix} 
        I_{n_1} & -\gamma_1 A^\top \\
        -\gamma_2 B & I_{n_2} - \gamma_1\gamma_2BA^\top
    \end{pmatrix}
\end{equation}
In zero-sum bilinear games, it has been shown that alternating gradient play have much better convergence properties in finite regret~\cite{bailey2019finite}. 


==> disturbanceReject.tex <==
\section{Bounded Noise Rejection}\label{sec:boundedNoise}
In this section we analyze how bounded noise affects both the convergence and transient behaviour of multi-agent learning dynamics for a general sum continuous game. We derive bounds on the maximum transient noise that the learning dynamics can handle without deviating from NE. In addition, we show that even when the noise cannot destablize learning dynamics, players to converge to Nash equilibrium that is offset from the original NE. 

\subsection{Bounded Noise in Finite Time Interval}
When noise is bounded and finite in time, we show that there exist step sizes which ensure stability of learning dynamics and that the transient behaviour of the dynamics do not leave the region of attraction of the Nash equilibrium.
\begin{assumption}[Bounded Noise] \label{ass:boundedNoise_finiteInterval}
There exists $\infty  > L > 0$, such that for all $k$, the total noise for all players, $g_k$, is bounded in norm by $L$, i.e., 
\[\norm{g^k}_2 \leq L, \quad \forall \ i \in [N], \ \forall\  k = 0, 1, \ldots, T. \]
\end{assumption}
We consider the uniform step-sizes derived in (CITE BEN) and show that there exists an inherent level of noise that the gradient dynamics is robust against.
\begin{theorem}[Step-sizes for bounded transient behaviour]\label{thm:boundedNoise}
Suppose that the gradient-learning dynamics for a $N$ player general sum continuous game is initialized wihtin region of attraction of a non-degenerate differential NE $x^\star$. I.e. $x_0 \in B_r(x^\star)$ and $\alpha >0$, where $r> 0$ is the largest region of attraction. If there exists $L < \alpha r$ that also satisfies assumption~\ref{ass:boundedNoise_finiteInterval}. Then noises whose 2 norm is bounded by $L$ will not destablize the gradient learning dynamics with uniform step size $\gamma = \frac{\alpha}{\beta}$.
\end{theorem}
\begin{proof}
From learning dynamics~\eqref{eqn:gradientUpdate} and noise model~\eqref{eqn:noiseModel}, we have
\[x^{k+1} = x^k - \Gamma w(x^k) -\Gamma g^k\]
Let $\tilde{g}(x) = x - \Gamma w(x)$, 
\[\norm{x^{k+1} - x^\star} = \norm{\tilde{g}(x^k) - \tilde{g}(x^\star) - \Gamma g_]k}  \]
We note that $\tilde{g}$ is differentiable in $x$, then from fundamental theorem of calculus, 
\begin{equation}
    \begin{aligned}
        \norm{\tilde{g}(x^k) - \tilde{g}(x^\star)}_2 & = \norm{\int_0^1D\tilde{g}(\tau x^k - (1-\tau)x^\star)(x_k - x^\star) d\tau }_2\\
        & \leq \sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}_2\norm{x_k - x^\star}_2
    \end{aligned}
\end{equation}
From this we can derive,
\[ \norm{x^{k+1} - x^\star}_2 \leq \sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}_2\norm{x^k - x^\star}_2 +  \norm{\Gamma g^k}_2 \]
$D\tilde{g}(x)  = I - \Gamma J(x)$. 
% Let $\alpha = \min_{x\in B_r(x^\star)} \min_{\lambda}\half\lambda(J(x) + J^T(x))$, and $ \beta = \max_{x \in B_r(x^\star)} \max_{\lambda} \lambda(J^T(x)J(x))$. 
Assuming that $\Gamma = \gamma I$ then 
\[\sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}\leq (1 - 2\gamma \alpha + \gamma^2 \beta ) \]
With $\gamma = \frac{\alpha}{\beta}$, the upper bound becomes $ (1 - \frac{\alpha^2}{\beta})$. Returning to the norm bound on $x^{k+1} - x^\star$, 
\[ \norm{x^{k+1} - x^\star}_2 \leq(1 - \frac{(\alpha)^2}{\beta})\norm{x^k - x^\star}_2 + \frac{\alpha}{\beta}L \]
Then for any $L < r\alpha$, $\norm{x^{k+1} - x^\star} \leq r$. 
% Let $L = C\norm{x_k - x^\star}$, then
% \[\norm{x_{k+1} - x^\star} \leq \big(1 - 2\gamma(\alpha + \half C) +  \gamma^2\beta\big)\norm{x_k - x^\star}\]
% Assuming we start within stabilizeable region around Nash equilibrium, $x^\star$, which has maximum radius $r$, $C \geq \frac{L}{r}$. Let $\bar{C} = \frac{L}{r}$, then 
% \[\norm{x^{k+1} - x^\star} \leq \big(1 - 2\gamma(\alpha + \half\bar{C}) +  \gamma^2\beta\big)\norm{x^k - x^\star}\]
% Assuming that $(\alpha + \half \bar{C})^2 < \beta$, a step size of $\gamma = \frac{\alpha + \half\bar{C}}{\beta}$ will give
% \[\norm{x^{k+1} - x^\star} \leq \big(1  - \frac{(\alpha + \half\bar{C})^2}{\beta}\big)\norm{x^k - x^\star}\]
% Which gives exponential convergence. The assumption that $\alpha + \half \bar{C} < \sqrt{\beta}$ is equivalent to 
% \[L < 2r(\sqrt{\beta} - \alpha)\]
% Finally, we note that convergence under this the step size only holds while $2\alpha + \frac{L}{\norm{x^k -x^\star}} < \sqrt{\beta}$. This gives a lower bound on the region of convergence,
% \[\norm{x^k - x^\star} >  \frac{L}{\sqrt{\beta} - 2\alpha }\]
% Which is within region of stability by assumption. Therefore we have that the learning dynamics under disturbance is guaranteed to converge to $B_{\bar{r}}(x^\star)$, where $\bar{r} = \frac{L}{\sqrt{\beta} - 2\alpha}$. 
\end{proof}

% \begin{theorem}[Step-sizes for bounded transient behaviour]
% \label{thm:boundedNoise}
% Suppose that the gradient-learning dynamics for a $N$ player general sum continuous game is initialized within region of attraction of a non-degenerate differential NE $x^\star$ in joint strategy space, i.e. $x_0 \in B_r(x^\star)$ and $\alpha > 0$~\eqref{eqn:minEigen}, where $r>0$ is the largest radius of region of stability. If the game Jacobian satisfies 
% \[\sqrt{\beta} \geq 2\alpha,\]
% and the noises on gradients satisfy Assumption~\ref{ass:boundedNoise_finiteInterval} for a finite constant $L$, and $L$ additionally satisfies 
% \begin{equation}\label{eqn:boundedNoise_criteria}
%     L < r(\sqrt{\beta} - 2\alpha).
% \end{equation}
% Then the uniform learning rate $\gamma = \frac{\alpha + \frac{L}{2r}}{\beta}$ ensures that the gradient learning is stable for all $N$ players.  
% \end{theorem}
% \begin{proof}
% From learning dynamics~\eqref{eqn:gradientUpdate} and noise model~\eqref{eqn:noiseModel}, we have
% \[x^{k+1} = x^k - \Gamma w(x^k) -\Gamma g^k\]
% Let $\tilde{g}(x) = x - \Gamma w(x)$, 
% \[\norm{x^{k+1} - x^\star} = \norm{\tilde{g}(x^k) - \tilde{g}(x^\star) - \Gamma g_]k}  \]
% We note that $\tilde{g}$ is differentiable in $x$, then from fundamental theorem of calculus, 
% \begin{equation}
%     \begin{aligned}
%         \norm{\tilde{g}(x^k) - \tilde{g}(x^\star)}_2 & = \norm{\int_0^1D\tilde{g}(\tau x^k - (1-\tau)x^\star)(x_k - x^\star) d\tau }_2\\
%         & \leq \sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}_2\norm{x_k - x^\star}_2
%     \end{aligned}
% \end{equation}
% From this we can derive,
% \[ \norm{x^{k+1} - x^\star}_2 \leq \sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}_2\norm{x^k - x^\star}_2 +  \norm{\Gamma g^k}_2 \]
% $D\tilde{g}(x)  = I - \Gamma J(x)$. 
% % Let $\alpha = \min_{x\in B_r(x^\star)} \min_{\lambda}\half\lambda(J(x) + J^T(x))$, and $ \beta = \max_{x \in B_r(x^\star)} \max_{\lambda} \lambda(J^T(x)J(x))$. 
% Assuming that $\Gamma = \gamma I$ then 
% \[\sup_{x \in Br(x^\star)} \norm{D\tilde{g}(x)}\leq (1 - 2\gamma \alpha + \gamma^2 \beta ) \]
% Let $L = C\norm{x_k - x^\star}$, then
% \[\norm{x_{k+1} - x^\star} \leq \big(1 - 2\gamma(\alpha + \half C) +  \gamma^2\beta\big)\norm{x_k - x^\star}\]
% Assuming we start within stabilizeable region around Nash equilibrium, $x^\star$, which has maximum radius $r$, $C \geq \frac{L}{r}$. Let $\bar{C} = \frac{L}{r}$, then 
% \[\norm{x^{k+1} - x^\star} \leq \big(1 - 2\gamma(\alpha + \half\bar{C}) +  \gamma^2\beta\big)\norm{x^k - x^\star}\]
% Assuming that $(\alpha + \half \bar{C})^2 < \beta$, a step size of $\gamma = \frac{\alpha + \half\bar{C}}{\beta}$ will give
% \[\norm{x^{k+1} - x^\star} \leq \big(1  - \frac{(\alpha + \half\bar{C})^2}{\beta}\big)\norm{x^k - x^\star}\]
% Which gives exponential convergence. The assumption that $\alpha + \half \bar{C} < \sqrt{\beta}$ is equivalent to 
% \[L < 2r(\sqrt{\beta} - \alpha)\]
% Finally, we note that convergence under this the step size only holds while $2\alpha + \frac{L}{\norm{x^k -x^\star}} < \sqrt{\beta}$. This gives a lower bound on the region of convergence,
% \[\norm{x^k - x^\star} >  \frac{L}{\sqrt{\beta} - 2\alpha }\]
% Which is within region of stability by assumption. Therefore we have that the learning dynamics under disturbance is guaranteed to converge to $B_{\bar{r}}(x^\star)$, where $\bar{r} = \frac{L}{\sqrt{\beta} - 2\alpha}$. 
% \end{proof}

\begin{remark}
Theorem~\ref{thm:boundedNoise} shows that gradient learning dynamics under small enough disturbance can still sustain stability. How small does the noise need to be is exactly characterized by the minimum eigenvalue of the symmetric game Jacobian and region of attraction. Furthermore, any bounded noise with small enough norm in a \emph{finite} time interval can alter neither convergence to Nash equilibrium nor joint strategy that is converged to originally.

% In particular for games with quadratic costs, the region of stability $r = \infty$, therefore any bounded noise such that
% \[\lim_{t \rightarrow \infty} \norm{g_k} = g\]
% will not affect the convergence behaviour of gradient descent dynamics.
\end{remark}
Specializing Theorem~\ref{thm:boundedNoise} to quadratic cost games, we can show that bounded noise that decreases to zero asymptotically does not affect convergence of player's strategies towards Nash equilibrium. 
\begin{corollary}[Bounded Noise for Quadratic Cost Continuous Games]
Consider an $N$ player general sum game whose costs satisfy Assumption~\ref{ass:quadGame}, and who has a non-degenerate differential NE. We assume that the gradient learning dynamics followed by players is corrupted by noise that satisfies Assumption~\ref{ass:boundedNoise_finiteInterval}. If the limiting behaviour of $g^k$ also satisfies
\[\lim_{k \rightarrow \infty} \norm{g^k} = 0,\]
then the uniform step size from Theorem~\ref{thm:boundedNoise}, $\gamma = \frac{\alpha}{\beta}$, ensures convergence of player strategies if the noiseless dynamics also converges.
\end{corollary}
\begin{proof}
This corollary follows from the fact that $J(x)$ is constant for all $x \in \real^{Nn}$. Quadratic cost games that satisfy Assumption~\ref{ass:quadGame} is composed of individual cost functions $f_i$ that are quadratic in $x_i$ and at most binlinear in $x_{-i}$ and $x_i$. Therefore $J(x)$ by definition is constant for all $x$. From definition of non-degenerate NE, $J(x^\star)$ is positive definite, therefore $J(x)$ is positive definite everywhere. Then the region of attraction of $x^\star$ is all of $\reals^{Nn}$, and therefore the step size from Theorem~\ref{thm:boundedNoise} holds for all of joint strategy space. 

The limiting behaviour of $\norm{g^k}$ suggests that for any $\delta > 0$, there exists positive integer $M$ such that $\norm{g^k} \leq \delta$ if $k \geq M$. From Theorem~\ref{thm:boundedNoise}, we have that any $\norm{x^k - x^\star} > 4 \frac{L}{\sqrt{\beta} - \alpha}$ will converge to within a ball of radius $r = 4 \frac{L}{\sqrt{\beta} - \alpha}$ around NE. Take $L = \delta$, since $J(x)$ is constant, $\alpha$ and $\beta$ are also constant. we have that for any $\delta > 0$, there exists positive integer $M$ such that any $\norm{x^k - x^\star} > 4 \frac{\delta}{\sqrt{\beta} - \alpha}$ will converge to a ball around $x^\star$ of radius $r =\frac{\delta}{\sqrt{\beta} - \alpha}$. Therefore the quadratic game converges asymptotically to NE $x^\star$. 
\end{proof}

\subsection{Bounded Noise with Unbounded Time Range}
Theorem~\ref{thm:boundedNoise} shows that convergence is possible when noise is bounded. We now consider when the noise magnitude can be arbitrarily large, but the noise itself is constant in time. In the case of quadratic cost games, we can show that while such constant noise does not affect convergence to NE, the point of convergence will be offset from the original NE by a magnitude proportional to the magnitude of input noise and step-size. 

\begin{theorem}[Fixed Adversarial Noise]
\label{thm:quadCostGame}
For quadratic cost games satisfying Assumption~\ref{ass:quadGame} with some noise that satsfies 
\[g^k, \ \lim_{k \rightarrow \infty} g^k = g\]
the gradient learning dynamics will converge for uniform step sizes given in Theorem~\ref{thm:boundedNoise}. Furthermore, the point of convergence, $x_{eq}$ will be offset from the original Nash equilibrium $x^\star$ by 
 \[x_{eq}  = x^\star  - J(x)^{-1}g\]
 where  $J(x)$ is the game Jacobian.
\end{theorem}

\begin{proof}
We consider a quadratic cost game satisfying Assumption~\ref{ass:quadGame} with constant adversarial noise $g$. For quadratic games, $D_if_i(x) = D_{i}^2f(x) x_i + \sum_{j \neq i}D_{ij}^2f_i(x)x_j + c_i$ for some constant vector $c_i \in \reals^{n}$. The learning dynamics can be re-written in terms of the constant game Jacobian as 
\[x^{k+1} = (I - \Gamma J(x))x_{k} - \Gamma(g + c).\]
Because the game is quadratic, $J(x) \succ 0$ holds for all $x$, the region of stability is all of strategy space, $r = \infty$. Then uniform step sizes from Theorem~\ref{thm:boundedNoise} applies $\frac{L}{2r} = 0$, such that $x^k \rightarrow x^{eq}$. The point of convergence can be solved for,
\[x^{eq} = (I - \Gamma J(x))x_{eq} - \Gamma (g + c)\]
Solving for $x^{eq}$ we obtain $x^{eq} = -J^{-1}(x)(c+g)$. 
Without disturbance, the Nash equilibrium is $x^\star = -J^{-1}(x)c$, therefore the new NE is offset from the orignal NE by $J^{-1}(x)c$.
\end{proof}

\subsection{Arbitrary Noise in Unbounded Time}






==> gameSetUp.tex <==
\section{Networked Continuous Game}
To facilitate the introduction of continuous games, we utilize the following notations. $[N] = \{1, 2, \ldots, N\}$ denotes a finite set of size $N$. We denote a closed and compact set as $\mc{X}$. For a function $f: \mc{X}^1 \times \ldots \times \mc{X}^N \rightarrow \reals$, $D_j(f)$ denotes its partial derivative with respect to domain $\mc{X}^j$, i.e. $D_j(f) = \frac{\partial f}{\partial x_j}$, and $D^2_{ij}(f) = \frac{\partial^2 f}{\partial x_j \partial x_i}$.
\subsection{Network Continuous Game}
We consider a continuous game played by $N$ players, where player $i$ has strategy variable $x^i \in \mc{X}_i$ with dimension $n_i$, and a continuous cost function given by $f_i: \mc{X}_1\ldots\times \mc{X}_N \rightarrow \reals$.
The goal of each player is to minimize its own cost function with respect to other players' strategies. 
\begin{equation}\label{eqn:individualoptimization}
    \underset{x^i \in \mc{X}}{\min} \ f_i(x^1, \ldots, x^N)
\end{equation}
The joint strategy profile is given by $x = \begin{bmatrix}x^1 & \ldots&x^N\end{bmatrix} \in \mc{X}_1\ldots \times \mc{X}_N$. A joint strategy is a \emph{local Nash Equilibrium} if no player can further reduce their cost within a local neighbourhood of their current action $(x^i)^\star$. 
\begin{definition}[Nash Equilibrium]
Given $N$ cost functions $\{f_i\}_{i=1}^N$, a strategy profile $x = \begin{bmatrix}x^1 & \ldots&x^N\end{bmatrix}$ is a Nash equilibrium if for each $i \in [N]$, 

\begin{align}
f_i(\ldots, (x^i)^\star, \ldots, (x^N)^\star) \leq f(\ldots, x^i, \ldots, (x^N)^\star), \\
\quad \forall \ x^i \in \mc{W}_i \notag
\end{align}
\end{definition}

In~\cite{mazumdar:2018aa}, it was shown that for almost all $N$ player continuous games, the set of non-degenerate differential Nash equilibria is generic among local Nash equilibria. 
\begin{proposition}[\cite{mazumdar:2018aa} Non-degenerate Differential Nash Equilibrium]
For almost all $N$-player games, a joint strategy $x \in \mc{X}$ is a local Nash equilibrium if and only if for all players' cost functions $f_1, \ldots, f_N$,
\[D_i f_i(x)  = 0 , \ D^2_{ii} f_i(x) > 0, \quad \forall \ i \in [N]\]
and 
\[\det(\begin{bmatrix}
D^2_{11}f_1(x) &  \ldots & D^2_{N1}f_1(x) \\
\ldots & \ddots &\ldots \\
D^2_{N1}f__N(x) & \ldots & D^2_{NN}f_N(x) \\
\end{bmatrix}) \neq 0\]
\end{proposition}

\subsection{Gradient-based Learning Dynamics}
In a non-cooperative setting, it is not obvious how and which Nash equilibrium players will converge to. We focus on learning algorithms where each player uses gradient-based information to minimize their cost function. Under an online learning scenario, a game is played repeatedly, with players determining their strategy based on the history of previous game play. In particular in gradient based learning dynamics, each agent updates their own strategy as
\begin{equation}\label{eqn:gradientUpdate}
    x^i(k+1) = x^i(k) - \gamma_i h^i(x^1(k), \ldots, x^N(k))
\end{equation}
where $\gamma_i$ is player $i$'s learning rate. We assume the players have \emph{oracle access} to its cost function gradient with respect to its own strategy. 
% The convergence of gradient based learning dynamics depends on the learning rate $\gamma_i$, we make the following assumption to ensure that all players' strategies converge. 
% \begin{assumption}
% Each player's cost function $f_i(x)$ satisfies
% \begin{equation}
%     \underset{j \neq i}{\sum^N} \norm{D^2_{ij}f_i}_2 \leq \norm{D^2_{ii}f_i}_2
% \end{equation}
% and each player's learning rate satisfies
% \begin{equation}
%     \gamma_i < \frac{2}{\underset{j = 1}{\sum^N} \norm{D^2_{ij}f_i}_2}
% \end{equation}
% \end{assumption}
In this paper, we consider the situation where player's access to its gradient is \emph{noisy}, i.e., 
\[h^i(x) = D_if_i(x) + g^i(w)\]
Where $g^i(w)$ models the additive noise that corrupts the gradient received by player $i$. When $g^i(w)$ is a zero mean stochastic process with finite variance, gradient-based learning converges irrespective of noise. Such a model however is restrictive in that it assumes inherent randomness in the noise, which does not generalize to adversarial disturbances. Instead, we model the noise as any continuous function with Lipschitz gradient bounds. 
\begin{equation}\label{eqn:noiseModel}
g^i: \reals^{m_i} \rightarrow \reals^{n_i}, \quad \norm{D_ig^i} \leq L
\end{equation}
By modelling noise as~\eqref{eqn:noiseModel}, we choose how the noise affects dynamics instead of dictating the trend of the noise by setting its expectation and variance. If there exists a model for the noise affecting the learning dynamics, but no assumptions can be made on what is causing the noise, ~\eqref{eqn:noiseModel} may prove to be more realistic than a stochastic model. \eqref{eqn:gradientUpdate} can be also used to model adversarial noises, in which an adversary may obscure player $i$'s gradient to destabilize the gradient based learning dynamics, and eventually cause failure to converge to a Nash equilibrium. 

When all players utilize gradient-based dynamics, the joint strategy $x$ will converge with appropriate step sizes under the following assumptions on each player's cost function $f$. 
\begin{assumption}[Cost Function Continuity]
For each player $i$, the cost function $f_i(x)$ is continuous in $x$. Furthermore, the quantity 
\[w(x) = \begin{bmatrix}D_1f_1(x) & D_2 f_2(x) & \ldots & D_N f_N(x)\end{bmatrix}\]
is $L-$ Lipschitz.
\end{assumption}
Different step sizes that guarantee multi-agent gradient learning convergence are given in~\cite{chasnov2019convergence}. We note that gradient learning always converges to a strict subset of Nash equilibria that is \emph{structurally stable} with respect to perturbations in gradient play~\cite{ratliff:2016aa}. In particular, we can consider just a specific type of Nash equilibria called \emph{non-degenerate differential Nash equilibria}. Let 
\[A(x) = I - \diag(\gamma_i)\begin{bmatrix}
D^2_{11}f_1(x) &  \ldots & D^2_{N1}f_1(x) \\
\ldots & \ddots &\ldots \\
D^2_{N1}f__N(x) & \ldots & D^2_{NN}f_N(x) \\
\end{bmatrix} .\]
The set of non-degenerate differential Nash equilibria forms an open dense subset of local Nash equilibria, and can be classified as either \emph{locally asymptotically stable} (LASE) or \emph{strict saddle point} (SSP)~\cite{mazumdar2018convergence}. 
We say that a Nash equilibria $x^\star$ is \emph{locally asymptotically stable} (LASE) if $A(x^\star)x^\star = x^\star$ and $\norm{A(x^\star)}_2 < 1$. Otherwise, we say that $x^\star$ is a a \emph{strict saddle point} (SSP) if $A(x^\star) x^\star = x^\star$ and there exists $\lambda \in \rho(A(x^\star))$ such that $|\lambda| > 1$. Gradient-based learning avoids strict saddle point equilibria. Intuitively, this implies that non-degenerate differential Nash equilibrium relaxes LASE criteria --- LASE imposes that $A(x^\star)$ itself must be positive definite, while non-degenerate differential Nash only requires the diagonal elements $D^2_{ii}f_i(x^\star)$ to be positive definite. 

We consider the situation where players are close to a LASE strategy. Around the equilibrium solution, the following linearized dynamics is used to approximate gradient learning dynamics. 
% If all players simultaneously update their strategies at time intervals $1, 2, \ldots k, k+1$ by taking the gradient of the joint strategy from previous game, the update can be written as 
\begin{equation}
    \begin{aligned}\label{eqn:discreteLTI}
        x(k+1) & = \bar{A}x(k)+ \bar{E} w(k)\\
        y(k+1) & = C x(k) \\
    \end{aligned}
\end{equation}
we shorten the notation to $x = \begin{bmatrix}x_1& x_2 & \ldots & x_N\end{bmatrix}^T$, $w = \begin{bmatrix}w_1& w_2 & \ldots & w_N\end{bmatrix}^T$.
\[\bar{A} = \begin{bmatrix}
I - \gamma_1Q^1_{11} & -Q^1_{12} & \ldots &-Q^1_{1N} \\ 
-Q^2_{21} & I - \gamma_2Q^2_{22} & \ldots & -Q^2_{2N}\\
\vdots & \ddots &   & \vdots \\
-Q^N_{N1} & -Q^N_{N2} & \ldots & I - \gamma_NQ^N_{NN}
\end{bmatrix}\]
\[\bar{E} = -\diag(\gamma_iS_i)\]
Where $ Q^k_{ij}  = D^2_{ij}f^k$, and $y(k) \in \mc{X}^n$ is performance criteria based on individual's strategies. This performance criteria can be a regret as taken in~\cite{agarwal2019online} in the example of deep reinforcement learning, or in the case of multi-agent tracking, the average position of all players.  
